Carbide: Highly Reliable Networks Through Real-Time Multiple Control Plane Composition

Achieving highly reliable networks is essential for network operators to ensure proper packet delivery in the event of software errors or hardware failures. Networks must ensure reachability and routing correctness, such as subnet isolation and waypoint traversal. Existing work in network verification relies on centralized computation at the cost of fault tolerance, while other approaches either build an over-engineered, complex control plane, or compose multiple control planes without providing any guarantee on correctness. This paper presents Carbide, a novel system to achieve high reliability in networks through distributed verification and multiple control plane composition. The core of Carbide is a simple, generic, efficient distributed verification framework that transforms a generic network verification problem to a reachability verification problem on a directed acyclic graph (DAG), and solves the latter via an efficient distributed verification protocol (DV-protocol). Equipped with verification results, Carbide allows the systematic composition of multiple control planes and realization of operator-specified consistency. Carbide is fully implemented. Extensive experiments show that (1) Carbide reduces downtime by 43% over the most reliable individual underlying control plane, while enforcing correctness requirements on all traffic; and (2) by systematically decomposing computation to devices and pruning unnecessary messaging between devices during verification, Carbide scales to a production data center network.

==> DV/azure-proof.tex <==
\section{Proof: Azure Example} \label{sec: azure-proof}
By definition, we have $\forall y \notin E_{out}(x), d_p(y = nil) = False$ ($E_{out}(x)$ consists of all outgoing edges for $x$). Then, we have the following derivation for this special case.
\begin{equation}
\begin{split}
    d_p(x) &= (\bigwedge_{y \in E_{out}(x)} d_p(y)) \wedge (N_p(x) = E_{out}(x)) \\
    d_p(src) &= (\bigwedge_{y \in E_{out}(src)} d_p(y)) \wedge (N_p(src) = E_{out}(src))\\
             &= (N_p(src) = E_{out}(src)) \wedge (\bigwedge_{y \in E_{out}(src)} (N_p(y) = E_{out}(y))\\
             &  \wedge (\bigwedge_{z \in E_{out}(y)} d_p(z)))\\
             &= \bigwedge_{y \neq nil} (N_p(y) = E_{out}(y))\\
             &= (y \neq nil) \Rightarrow (N_p(y) = C(y))
\end{split}
\end{equation}

==> DV/backup.tex <==
\richard{conditional verification}



==> DV/codes.tex <==
% Outline items:
% 
\begin{proposition}
Assume source broadcasts the mapping $f$ from (switch, packet-space) to DFA-state, a node $N$ can locally compute backups: for each packet-space $s$, it can locally compute its state, i.e., $f(N, s)$, and forward the packet to a next-hop $M$ satisfying $f(M, s) = f(N, s).\sigma(M)$ where $\sigma$ is the transition function in DFA.
\end{proposition}

% FIXME: the CPs in the following alg should also record the potential state in g-DFA (otherwise, it needs the order to form a sequence)
\begin{algorithm}[h]
    \SetAlgoLined
    \KwData{vFIBs (with attribute CP to records all entries from different CPs, and attribute S to label state);  assume the priorities have been removed, and every entry match on a header space}
    \KwResult{Violation Table $\{S.T\}_{S \in cDFA}$}

    \ForEach{$S \in cDFA$} {
        \ForEach{$entry \in S.node.vFIBs$} {
            \If{$entry.action$ doesn't follow cDFA}{
                $hs = entry.match$\;
                $cps = dict((S.node, entry.CP))$\;
                \eIf{$S \in $ Coverage-set} {
                    Directly announce $cps$ back to source\;
                }{
                    $S.T.insert((``HS" = hs, ``CPs" = cps))$\;
                }
            }
        }
    }
    \ForEach{$S \in DFA$ following reversed topological order} {
        \ForEach{$e1 \in S.node.vFIBs$} {
            \ForEach{$e2 \in S'.T$ where  $S' \in S.next(e1.action)$ and $e1.action$ follows cDFA} {
                $hs = e1.match \wedge e1.rev(e1.modify \wedge e2.hs)$\;
                $cps = dict((S.node, e1.CP)) + e2.cps$\;
                \If{$hs \neq \emptyset$ and $cps$ follows gDFA}{
                    $S.T.insert((``HS" = hs, ``CPs" = cps)$
                }
            }
        }
    }
    
    source node needs to solve a SAT problem: for packet space $ps$, find a CP-composition plan $cps$ satsifying:
    $\nexists e \in Src.T, ps \wedge e.hs \neq empty$ and $e.cps \subseteq cps$
\caption{Centralized Verification (CDT) for Composition}
\end{algorithm}

% TODO: rename, like next() -> dfa_next()

\begin{algorithm}[h]
    \SetAlgoLined
    \KwData{FIB}
    \KwResult{Violation Table Entries \{$S.H$\}}

    \ForEach{$S \in DFA$} {
        $S.H = \emptyset$\;
        \ForEach{$entry \in S.node.FIB$} {
            \If{$S.next(entry.action) \notin DFA$}{
                $S.H = S.H + entry.match$\;
            }
        }
    }
    \ForEach{$S \in DFA$ following reversed topological order} {
        \ForEach{$entry \in S.node.FIB$} {
            $S' = S.next(entry.action)$\;
            $S.H = S.H + entry.match \wedge S'.H$\;
        }
    }
\caption{Centralized Verification (CDT)}
\end{algorithm}

\begin{algorithm}[h]
    \SetAlgoLined
    \KwData{$N.FIB$}
    $N.SFIB = N.VFIB = N.AFIB = \emptyset$\;
    \ForEach{$S \in DFA(N)$} {
        \ForEach{$entry \in N.FIB$} {
            \If{$S.in \wedge entry.ingress \neq \emptyset$} {
                $N.SFIB = N.SFIB + (S, entry)$\;
            }
        }
    }
    \ForEach{$entry \in N.SFIB$} {
        \eIf{$entry.state.next(entry.action) \in DFA$)}{
            $N.AFIB = N.AFIB + entry$\;
        } {
            $N.VFIB = N.VFIB + entry$\;
        }
    }
\caption{Distributed Verification (DDT) Local Part}
\end{algorithm}

\begin{algorithm}[h]
    \SetAlgoLined
    \KwData{$N.VFIB$}
    \ForEach{$entry \in N.VFIB$} {
        $nodes = \emptyset$\;
        \ForEach{$S \in DFA$} {
            \If{$S.next(N) = entry.state$ and $S.node \in entry.ingress$} {
                $nodes = nodes + S.node$\;
            }
        }
        Send $\{entry\}$ to $nodes$\;
    }
\caption{Distributed Verification (DDT) Msg Initialization}
\end{algorithm}

\begin{algorithm}[h]
    \SetAlgoLined
    \KwData{$Msg$}
    \KwResult{Local Violation Table Entries \{$N_i.H$\}}
    $update = \emptyset$\;
    \ForEach{$mentry \in Msg$} {
        \ForEach{$entry \in N.AFIB$} {
            \If{$mentry.state \in entry.state.nexts(entry.action)$} {
                $entry' = entry$\;
                $entry'.match = entry.match \wedge mentry.match$\;
                $entry.match = entry.match - entry'.match$\;
                $update = update + entry'$
            }
        }
    }
    $N.VFIB = N.VFIB + update$\;
    \ForEach{$entry \in update$} {
        $nodes = \emptyset$\;
        \ForEach{$S \in DFA$} {
            \If{$S.next(N) = entry.state$ and $S.node \in entry.ingress$} {
                $nodes = nodes + S.node$\;
            }
        }
        Send $\{entry\}$ to $nodes$\;
    }
\caption{Distributed Verification (DDT) Msg Response}
\end{algorithm}

\begin{algorithm}[h]
    \SetAlgoLined
    \KwData{Incoming $Msg$, $NMsg$}
    \KwData{Local State $N.SFIB$}
    \KwResult{Local Violation Table Entries \{$N_i.H$\}}
    initialization $record = \{entry: (State: Rejecting, Match: *, Action: \_)\}$ (It's a small trick to unify alg3 into alg4)\;
    $records = records + Msg$\;
    Specially, there can be cancel messages $NMsg$\;
    $records = records - NMsg$\;
    $N.NVFIB = \emptyset$\;
    \ForEach{$mentry \in records$} {
        \ForEach{$entry \in N.SFIB$} {
            \If{$mentry.state \in entry.state.nexts(entry.action)$} {
                $entry' = entry$\;
                $entry'.match = entry.match \wedge mentry.match$\;
                $N.NVFIB  = N.NVFIB + entry'$
            }
        }
    }
    The messages sent should be consistent with the $N.VFIB$\;
    \ForEach{$entry \notin N.VFIB$ and $entry \in N.NVFIB$}{Send messages for $entry$}
    \ForEach{$entry \in N.VFIB$ and $entry \notin N.NVFIB$}{Send cancel messages for $entry$}
    $N.VFIB = N.NVFIB$\;
\caption{Dummy DDT with Incremental Update}
\end{algorithm}

\begin{algorithm}[h]
    \SetAlgoLined
    \KwData{Incoming $Msg$, $NMsg$}
    \KwData{Local State $N.SFIB$}
    \KwResult{Local Violation Table Entries \{$N_i.H$\}}
    $update = \emptyset$\;
    \ForEach{$mentry \in Msg$} {
        \ForEach{$entry \in N.SFIB$} {
            \If{$mentry.state \in entry.state.nexts(entry.action)$} {
                $entry' = entry$\;
                $entry'.match = entry.match \wedge mentry.match$\;
                $update  = update + entry'$
            }
        }
    }
    \ForEach{$entry \notin update$}{Send messages for $entry$}
    And do the similiar thing for NMsg\;
\caption{Smart? DDT with Incremental Update}
\end{algorithm}


==> DV/requirements-old.tex <==
\subsection{Verification Requirements Specification}
\richard{complete grammar for V2 and claim very generic grammar for FSD}
% we don't introduce performance metric
% clarify the difference among 4 packet spaces of (1) user requirements; (2) FIB entries; (3) path-construction function; (4) verification results. 

\begin{figure}
\ttfamily
\small
\begin{tabular}{r L  l}
       h & \in & packet headers
    \\ f & \in & header fields
    \\ v & \in & header field values
    \\ label & \in & device labels
    \\ 
    \\ pkt\_space & := &  (h.f=v)
    \\ & | & (pkt\_space [$|$, \&] pkt\_space)
    \\ & | & !pkt\_space
    \\
    \\ path & := & $\&$ $|$ $\$$ % a sequence of devices, but
    \\ & | & [label] path % also considered as a set of devices
    \\
    \\ path\_set & := & $DP^A(p)$
    \\ & | & $DP^M(p)$
    \\ & | & Regex
    \\ & | & (path\_set [$\wedge$, $\vee$] path\_set)
    \\ 
    \\ predicates & := & path\_set set\_comparison path\_set
    \\ & | & (predicates [$|$, \&] predicates)
    \\ & | & !predicates
    \\
    \\ requirements & := & predicates
    \\ & | & $\forall$ p $\in$ pkt\_spec, requirements
    % \\ & | & $\exists$ p $\in$ pkt\_spec, requirements
    % FIXME: do we really need "exists"? Disjoint path also use Pt \in DP
    \\ & | & (requirements [$|$, \&] requirements)
    \\
    \\ Regex & := & ...
\end{tabular}
\normalfont
	\caption{\small{\ReqLang specification.}}\label{fig:dv-grammar}
\reducespace
\end{figure}

% V output: packet space
%   input: (1) path-construction function (from DP model),  
%          (2) requirements (defined in this section)
%
% Requirements:
%   (1) labels of devices (and precomputation)
%   (2) Regex as a set of paths (safety-set and coverage-set)
%   (3) packet space
%   (4) logic expressions

\DistVeri provides a formal framework for operators to specify verification requirements. First, operator specify one or multiple packet space. Then,  operator specify predicts consisting of set of paths, set operations and logical operations. The set of paths can be: (1) $DP^A(p), DP^M(p)$ where $p$ belongs to a packet space and (2) a set $\mathcal{P}$ of paths specified by regular expression (Regex).

\richard{introduce local switching (for backup next-hop)}

\begin{itemize}
    \item \textbf{Labels for devices}: Requirements are specified for a set of network devices. Each network devices can have multiple labels. A label can be its ip addresses, identifier, tier in a fat tree topology, and probably represent whether it is a load-balancing servers. 
    \item \textbf{Regex as a set of path}: A regular expression can specify a set of paths where each paths is a sequence of devices and optionally a loop/end-sign. \DistVeri\ uses Pearl-like Regex grammar but extends it with $[label]$ referring to a device with $label$.
    \item \textbf{Packet space}: A packet space is specified as a set of predicts of packet attributes. It refers to a set of packets whose attributes satisfy this set of predicts.
    \item \textbf{Predicates}: it include (1) set of paths, (2) logic operations $\{\forall, \exists, \&, |\}$ and (3) set operations $\{\wedge, \vee, \subset, \supset, =\}$.
\end{itemize}

\shen{redundant..}
The requirements is specified as logic predicts using grammar shown in Figure~\ref{fig:dv-grammar}. Besides logic operations and set operations, this grammar mainly uses the following variables: header/packet-space, $DP^A$, $DP^M$ and a set $\mathcal{P}$ of paths represented by regular expressions. One syntax sugar for Regex is $[label]$ which allows operator to specify a group of devices with the $label$. 
% a coverage-set can be specified with a regex and \supset; notice the regex can be a set of path-prefixes

Although regular expression only can specify a constant set of paths, operator can extend it by introducing additional label to devices and specify paths using label. Taking the shortest-path requirements as an example, for a single source, it can be specified with two steps: (1) label every device with the minimal distance from source; (2) specify the regular expression capturing all shortest-path using $[label]$ grammar.

{\tiny
Reachability:
\begin{align}
& \forall d \in D, p \in pkt(dst: d), \\
& \emptyset \neq DP^M(p) \subseteq \mathcal{P} = (. *) [d]
\end{align}

\richard{assume we know all multicast receivers}

Multicast reachability:
\begin{align}
& \forall vip \in D, p \in pkt(dst: vip), \\
& \forall dip, [dip] \wedge [vip] \neq \emptyset, \\
& DP^M(p) \wedge (. *) [dip] \neq \emptyset 
\end{align} % two choices to specify: (1) intersection of path sets and (2) coverage-set

Reverse path:
\begin{align}
& \forall s \in S, d \in D, p_1 \in pkt(src: s, dst: d), p_2 \in pkt(src: d, dst: s),\\
& DP^M(p_1) = \lnot DP^M(p_2)
\end{align}

Load-balancing:
\begin{align}
& \forall d \in VIP, p \in pkt(dst: d),\\
&  DP^A(p) \supseteq \mathcal{P} = (. *) [AIP]
\end{align}

Shortest-path (constant length k):
\begin{align}
& \forall d \in D, p \in pkt(dst: d), \\
& DP^A(p) \subseteq \mathcal{P} = [D0] [D1] \dots [Dk]
\end{align}

Disjoint-paths:
\begin{align}
& \forall p_1, p_2 \in PS, p_1 \neq p_2,\\
& \forall Pt_1 \in DP^A(p_1), Pt_2 \in DP^A(p_2),\\ 
& Pt_1 \wedge Pt_2 = \emptyset
\end{align}
}

\shen{Goal: output of V()}
The objective of verification is to compute: for which set of packets, the paths constructed by the given datapath DP satisfy user requirements. 

\subsection{FIB-State Distributed Verification}
\shen{V1()} FSD can handle generic requirements. 
% We design V to consist of a sequence of logical expressions based on paths,  Claim a generic framework is to distributed FIB collection.
// FB requirements: (1) reachability; (2) failure handling; (3) traffic engineering; (4) label of addresses; (5) transformation; (6) originate; (7) propagation. 
// reverse path requirements 

\shen{think-the-order: defend BGP path collection}
// Defense: the distributed verification is fundamentally collecting paths;
One may concern existing control-plane like BGP and OSPF already collected paths, and predicts can be directly verified on their paths. // the paths collected by BGP can be wrong since they can be buggy (with emerging of white-box switches, there are different versions of software constantly changing). 

==> DV/writeup-old.tex <==
% 1. collect high-level components for technical content
% 2. topic sentence for each components
% 3. collect the attack/defend
% 4. re-organize them into paragraphs

% TODO: reorganize datapath-model para (entry, FIB, DP)

\richard{Consider all header space entering at Source}

% Component: DV
\richard{Distributed verification is a core component of Carbide. At the same time, DV can be a generic technique which can be used in other settings (...). To design a DV framework, the high level components. Together, i.e,, they allow each node to make local decisions.} Distributed Verification (DV) is a core component of Carbide. At the same time, DV can be a generic technique which can be used in other settings like Microsoft's Azure (cite SIGCOMM'19).
To design a DV framework, the high level components are: % (1) static DFA construction, (2) local verification and (3) update agent. 
\shen{what are the key components}
% FIXME high level components?
Together, i.e,, they allow each node to make local decisions.

% Component: Datapath
\richard{// Model and Requirements // Datapath model Verification is for a given datapath (FIB at each switch). In this DV model, // Make clear single CP, given stable each CP consists of an FIB at each node. Denote datapath DP. Lower layer can be LB or robustness. ... generic group FIB model ANY. // mention multicast will be handled differently }
Verification is for a given datapath (FIB at each switch). In this DV model, each CP consists of an FIB at each node. Here we describe DV for each single stable CP and the denote its datapath as DP. 
\richard{Notations// example}
\begin{definition}
The datapath $DP = \{FIB^i\}_{i = 1}^{n}$ where $FIB^n$ represents the FIB at node $n$ and $N$ is the set of nodes in network.
\end{definition}
% Sub-Component: FIB
\richard{The FIBs of the switches of the network construct paths (handle issue of loops, drops). Explain/clarify LB/robustness.}
We take a generic group FIB model with two logic operations ANY and ALL. A FIB entry takes action to forward packet to a group of next-hops. With ANY and ALL respectively, it forwards a packet to a single next-hop or multicasts a packet to all of next-hops. Such group model allows load-balancing and back-up paths for robustness. Keywords ANY and ALL handle the unicast and multicast respectively.
\begin{definition}
A $FIB = \{entry_1, \dots, entry_k\}$ where $k = |FIB|$
% and  the cardinality of $FIB$ is the number of entries
. Each $entry$ is in the form of $(match, ANY/ALL \; in \; NH)$. A packet hits on $match$ will be forwarded to ANY/ALL next-hops in the group $NH$.
\end{definition}
\shen{$NH$ can be a singleton}

% Component: Paths
\richard{Introduce notation for the paths (depends on what we need later; the whole set of paths, a function mapping from a packet to a set of paths, packet space??) …}
The FIBs of the switches of the network construct paths. 
% (handle issue of loops, drops).
Each FIB forwards a packet according to its header (and ingress port). Together, they provide a group of paths for a header. 
\begin{definition}
The paths constructed by a $DP$ is notated as $F_P(DP)$. It is a function mapping a packet $h$ to a set $P$ of available paths, i.e., $F_P(DP): h \mapsto P$.
\end{definition}
% Clarify why we don't capture the following semantics in definition
% A reason is they doesn't affect the requirements we are going to verify
The $DP$ unicasts a packet with header $h$ to a single path in $F_P(DP)(h)$ when all FIBs use logic ANY; Otherwise, the $DP$ multicasts a packet with header $h$ to a set of paths belonging to $F_P(DP)(h)$.
% Explain/clarify LB/roubustness
DV doesn't verify the implementation of FIB: taking load-balancing as an example, DV only verifies logic, which should be ANY, in FIBs and the groups of next-hop; one implementation is deciding the next-hop for a packets using hash-functions, which is agnostic to DV.

% Component: V()
\richard{// Verification requirements specification // the slide is not there The objective of verification is to decide whether the paths constructed by the given datapath DP are acceptable. Let V() the function? (V ( path( ) ) == false; handle the case that V verifies the set of paths for robustness.}
The objective of verification is to decide whether the paths constructed by the given datapath DP are acceptable. Let $V$ be a verification function. 
\begin{definition}
A verification function $V$ takes as input the $F_P(DP)$ and outputs $true$ or $false$ representing the network satisfying requirements or not, i.e., $V: F_P(DP) \mapsto \{true, false\}$
\end{definition}
% REDO the following part
% FIXME should we define a P_r for each H
Assume $P_r$ is the set of all requirement-compliant paths for headers in $H$, one basic requirement can be the expressed as: $\forall h \in H, F_P(DP)(h) \subseteq P_r$. It specifies the paths that can be available, which guarantees basic "safety" like loop-freeness and black-hole free. % FIXME: what is "safety"?
Furthermore, to provide load-balancing and robustness, the $DP$ also requires all paths should be available. It can be expressed as $\forall h \in H, F_P(DP)(h) = P_r$.

% Component: Automata
\richard{// To compactly specify V, we use automata/logic. // attack We consider V which can be specified using automata/logic. { defend missing cases;  } , as previous work (Propane). The previous work uses automama to specify requirements for construction and we use them here for verification. We further extend from only automama to include logic (what?)}
We consider $V$ which can be specified using automata and logic. The automata captures every single path, as previous work (Propane), but has difficulty on expressing the combination of paths and their relationship. The previous work uses automama to specify requirements for construction and we use them here for verification. 
We further extend from only automama to include two logic: $\subseteq$ and $=$. Previous work (Propane) uses $\subseteq$ by default and doesn't capture the next-hop groups using automata. DV takes the extension to verifies the next-hop groups used by FIB actions.

\richard{Specifically, ……}
Specifically, the "safety" is verified by logic $\subseteq$, i.e., each FIB only forwards packet to a requirement-compliant next-hop. The "availability" (for load-balancing or robustness) is captured by $=$, i.e., each FIB should provide all requirement-compliant next-hops.
% TODO: can we make verification more fine-grained

% Component: F-DFA
\richard{Automata can be compactedly converted to DFA, Specify using standard approach. … some details and notations}
% FIXME: all aforementioned automatas are actually DFAs...
Automatas can be compactedly converted to a single minimal DFA  using standard approach (cite DFA-product, DFA-minimization). 
\begin{definition}
The DFA is a tuple $(S, \Sigma, F, s_0, \sigma)$. $S$ is the set of states, $\Sigma$ is the alphabet. The initial state is $s_0$, $F_i$ is the set of accepting / final states, $\sigma: S \times \Sigma \rightarrow S$ is the transition function.
\end{definition}
As previous work (Propane), this DFA captures all requirement-compliant paths. A packet has a state $s_p$ starting from the initial state $s_0$. When FIBs forward it to a next-hop to node $n$, the state $s_p$ takes transition to become $\sigma(s_p, n)$; When $\sigma(s_p, n) \notin S$, the function verification $V$ should return $false$.

% Component: CDT (State) (Transition?)
\richard{// Distributed Verification A naive approach is centralized verification, which has access to the global DFA and the FIBs of all devices, but this is not ...}
% including State-FIB, Accept-Table, Violation-Table
A naive approach is centralized verification, which has access to the global DFA and the FIBs of all devices, but this is not ...

% Component: DDT
% including Back-Propagation
The complete DV is decomposed to distributed nodes where each node has three main components: (1) static DFA construction, (2) local verification and (3) update agent.

\subsection{Scalability}
\shen{Component: Abstract-Topo}
% Here a DP is not necessarily to be a real network, it can also be a virtual abstract DP for scalability concern. Nowdays a datacenter network ha millions of nodes which are configured using templates (cite FB). Those templates gives FIBs on an abstract view of topology. % FIXME is that true?
% The datacenter will keep the real network consistent with templates, and thus DV only verifies templates.



\subsection{Main Results}
\begin{proposition} % coverage-set P_C, Safety-set P_S
A requirement in form of $\forall h \in H, P_C \subseteq P_h \subseteq P_S$ is local verifiable iff $P_C = P_S$
\end{proposition}
\begin{proposition} % TODO formalize the mapping from node to state
A local verifiable requirement is satisfiable iff each node has at most 1 state in DFA.
\end{proposition}


==> DV/writeup.tex <==
\DistVeri\ is a core component of \system. At the same time, it
can be a generic technique which can be used in other settings~\cite{}\qiao{TBA}.
The distributed verification framework includes four key components: data-plane
model (Section~\ref{sec:dv-dpmodel}), verification requirement specification
(Section~\ref{sec:dv-grammar}), \shen{FSD} and distributed verification protocol
(Section~\ref{sec:dv-protocol}).

\begin{figure}[t]
\setlength{\abovecaptionskip}{0.1cm}
\setlength{\belowcaptionskip}{-0.cm}
\centering
\includegraphics[width=0.6\columnwidth]{images/dv-example-topology-v0.pdf}
\caption{\small{A running example.}}
\label{fig:dv-example-topology}
\reducespace
\vspace{-1em}
\end{figure}

\subsection{Data-plane Model}
\shen{DP and FIBs}
Verification is for each single control plane $CP_i$. At a certain time (assume the CP is stable), the forwarding behavior of a $CP_i$ is determined by its data-plane (notated as DP). A DP consists of Forwarding Information Base (FIB). Consider a network with $n$ forwarding devices (and a lot of other devices like hosts), each forwarding device has been labelled with an unique id $j$ from 1 to $n$. \DistVeri models the data plane generated by $CP_i$ as $\{FIB_i^j\}_{1 \leq j \leq n}$. 

\shen{header-space/packet-space should be introduced earlier}

\begin{figure}[t]
\centering
\includegraphics[width=1\columnwidth]{images/dv-fib.png}
\caption{\small{A Generic Abstraction of FIB.}}
\label{fig:dv-fib}
\reducespace
\end{figure}

\system\ takes a generic representation of FIB as shown in Figure~\ref{fig:dv-fib}. A $FIB_i^j$ is a table where each entry associates a header space ~\cite{kazemian2013real} to an action. An action consists of a set of next hops ~\cite{jayaraman2019validating} with a model (in two) and a modification function of packet header. // modification function and its reverse function in HSA. // Clarify: when user specify requirements for a packet-space, we only verify packets whose original header belong to this space.
A forwarding device processes packets using FIB by two steps: first, it finds the header space this packet belongs to // clarify HSA header spaces are disjoint; second, it applies modification function to packet header and forward it to other devices according to the set of next hops and its model.
// \DistVeri is oblivious of hardware realization. // allow, but don't verify local state of switch 

Here are descriptions for the two types:
\textbf{Anycast model}: a set of next hops can be used in anycast model with keyword $ANY$. This model specifies the non-determinitic forwarding behavior, \ie, a device can forward packets to any next hop in this set. A device can forward packets to different next hops even they share the same packet header. 
// examples: fault-tolerance/roubustness, anycast, load-balancing. \textbf{Multicast model}: a set of next hops can be used in multicast model with keyword $ALL$. This model specifies the determinitic forwarding behavior, \ie, a device always multicast packets to all next hops in this set.

\shen{CP-adapter}
\system\ allows adapter to extract FIB from specific control-planes. This design has two major advantages: (1) it provides future-proof, \eg, a novel control plane may use completely different model of FIB and operator still can use it by providing an adapter; (2) it allows us to pre-verify the forwarding behavior after some update, \eg, a CP may have some backup paths (\eg fast rerouting) not installed in DP and an adapter can extract those paths from CP. Those backup paths can be naturally captured by a set of next hops using anycast model. Although the implementation may always use primal next-hop, it is oblivious to our abstract FIB model. // clarify access control lists (ACLs)

\shen{Single-path definition}
A generic $P$ consists of a sequence of devices and optional end-sign $\$$ or loop-sign $\&$. A path with loop can be notated as a sequence while last two elements are a device  appeared before and the loop-sign $\&$. A path with drop can be notated as a path end with end-sign $\$$. // don't distinguish it is dropped, received or forwarded outside the topology; this only specifies this packet won't be forwarded to any device in topology. // clarify: a path w/o end-sign is a prefix of path; the last device can continue forward the packet while its behavior is not specified yet.

\shen{path-construction function}
The FIBs of the switches of the network construct paths. The path-construction is formalized as two functions mapping from a packet to a set of paths. The first function is \textbf{non-deterministic} \richard{this concept can be funny} forwarding path function $DP^A(h)$: assume a packet go through one path (in the set) in anycast model (clarify robustness), but other packets sharing the same header $h$ may go through different paths (clarify LB). Taking FB backup path requirements as an example, those require backup path are also provided which can be captured by group table using anycast model. // connect to the CP-adapter which extracts additional FRR info. The second function is the \textbf{deterministic} $DP^M(h)$ gives the set of paths that every packet taking header $h$ will traverse through where each duplication traverse one path. \shen{we don't verify the mix of them}  
Those two functions captures a bunch of useful verification requirements (reachability, loop-free, shorest-path, etc.). To avoid unnecessary complexity, \DistVeri\ doesn't consider other behaviors.

\subsection{Verification Requirements Specification}
\richard{complete grammar for V2 and claim very generic grammar for FSD}

\shen{claim generic grammar for FSD} Conceptually, \DistVeri\ are collecting all paths from FIBs and accepts generic verification requirements. Operator can write program to verify predicate on paths collected from FIBs. It can use first-order logic, set-operations, logic-operations and etc. This almost includes anything fitting into Turing-machine.

\begin{figure}
\ttfamily
\small
\begin{tabular}{r L  l}
       h & \in & packet headers
    \\ f & \in & header fields
    \\ v & \in & header field wildcard match
    \\ label & \in & device labels
    \\ 
    \\ pkt\_space & := &  (h.f: v)
    \\ & | & (pkt\_space [$|$, \&] pkt\_space)
    \\ & | & !pkt\_space
    \\
    \\ path & := & $\&$ $|$ $\$$ % a sequence of devices, but
    \\ & | & [label] path % also considered as a set of devices
    \\
    \\ path\_set & := & $DP^A(p)$
    \\ & | & $DP^M(p)$
    \\ & | & Regex
    \\ & | & (path\_set [$\wedge$, $\vee$] path\_set)
    \\ 
    \\ requirements & := & $\forall$ p $\in$ pkt\_spec, path\_set [$\subset, =$] path\_set
    \\
    \\ Regex & := & ...
\end{tabular}
\normalfont
	\caption{\small{\ReqLang specification.}}\label{fig:dv-grammar}
\reducespace
\end{figure}

\shen{specify grammar for V2()}
Without losing generality, \DistVeri\ is optimized for a subset of verification requirements using grammar shown in Fig~\ref{fig:dv-grammar}. Here are some examples: 

{\tiny
Reachability:
\begin{align}
& \forall d \in D, p \in pkt(dst: d), \\
& \emptyset \neq DP^A(p) \subseteq \mathcal{P} = (. *) [d]
\end{align}

Way-pointing:
\begin{align}
& \forall p \in pkt(), \\
& \emptyset \neq DP^A(p) \subseteq \mathcal{P} = (. *) [W] (. *)
\end{align}

Load-balancing:
\begin{align}
& \forall d \in VIP, p \in pkt(dst: d),\\
&  DP^A(p) \supseteq \mathcal{P} = (. *) [AIP]
\end{align}

Shortest-path (constant length k):
\begin{align}
& \forall d \in D, p \in pkt(dst: d), \\
& DP^A(p) \subseteq \mathcal{P} = [D0] [D1] \dots [Dk]
\end{align}
}

Formally, those requirements are specified following 3 steps:
\begin{itemize}
    \item \textbf{Path-set provided by FIBs}; To select a path-set provided by FIBs, operator first specifies a \textbf{packet space} with predicates of packet attributes. Then, by applying a packet in such packet space to path-construction function $DP^A$, operator selects a path-set.
    \item \textbf{Path-set specified by operator}: Operator can construct path-set using an extended \textbf{regular expression} (Pearl-like Regex grammar). A complete path should end with a end-sign $\$$; otherwise, it represents a path-prefix. This extended grammar provides $[label]$ refers to a device with $label$. A \textbf{device label} is generic and it can be ip addresses, identifier, tier in a fat tree topology, and probably represent whether the device is a load-balancing servers. 
    \item \textbf{Predicate on path-sets}: For a pair of path-sets provided by FIBs and specified by operator respectively, operator can specify a predicate using set operations $\{\subset, =\}$. Operator can specify multiple predicates and combine them using logic operations $\{|, \&, !\}$. Noticing operator may specify path-prefix in path-set $\mathcal{P}$, it takes a loose constraint:  when requiring $DP^A(p) \subset \mathcal{P}$, $\mathcal{P}$ is considered as including all path with such prefix; when requiring $\mathcal{P} \subset DP^A(p)$, $DP^A(p)$ just need one path with such prefix. \shen{clarify this part; maybe just remove it...}
\end{itemize}
As a summary, those requirements can always be written in form of: $\forall p \in hs_i, DP^A(p) \neq \emptyset, \mathcal{P}_c \subseteq DP^A(p) \subseteq \mathcal{P}_s$. Operator may not directly specify $\mathcal{P}_c$ and $\mathcal{P}_s$, but they can be statically computed from path-set specified by operator.

\richard{introduce local switching (for backup next-hop)}
% a coverage-set can be specified with a regex and \supset; notice the regex can be a set of path-prefixes

Although a regular expression only can specify a constant set of paths, operator can extend it by introducing additional label to devices and specify paths using label. Taking the shortest-path requirements as an example, for a single source, it can be specified with two steps: (1) label every device with the minimal distance from source; (2) specify the regular expression capturing all shortest-path using $[label]$ grammar.

\shen{this subset of requirements allow verifying each path in isolation; that's why it is fast}
\textbf{Limitations}: this subset doesn't include requirements that will cause combinatorial explosion, \ie, requiring predicates on multiple paths provided by FIBs. Here are examples:
{\tiny
\richard{assume we know all multicast receivers}
Multicast reachability:
\begin{align}
& \forall p \in PS, dip \in M_{rec}, \\
& DP^M(p) \wedge (. *) [dip] \neq \emptyset 
\end{align} 

Reverse path:
\begin{align}
& \forall s \in S, d \in D, p_1 \in pkt(src: s, dst: d), p_2 \in pkt(src: d, dst: s),\\
& DP^M(p_1) = \lnot DP^M(p_2)
\end{align}

Disjoint-paths:
\begin{align}
& \forall p_1, p_2 \in PS, p_1 \neq p_2,\\
& \forall Pt_1 \in DP^A(p_1), Pt_2 \in DP^A(p_2),\\ 
& Pt_1 \wedge Pt_2 = \emptyset
\end{align}
}

\shen{Goal: output of V()}
The objective of verification is to compute: for which set of packets, the paths constructed by the given datapath DP satisfy user requirements. 
% we don't introduce performance metric
% clarify the difference among 4 packet spaces of (1) user requirements; (2) FIB entries; (3) path-construction function; (4) verification results. 
% 
% V output: packet space
%   input: (1) path-construction function (from DP model),  
%          (2) requirements (defined in this section)

\subsection{FIB-State Distributed Verification}
\shen{V1()} FSD can handle generic requirements. 
% We design V to consist of a sequence of logical expressions based on paths,  Claim a generic framework is to distributed FIB collection.
// FB requirements: (1) reachability; (2) failure handling; (3) traffic engineering; (4) label of addresses; (5) transformation; (6) originate; (7) propagation. 
// reverse path requirements 

\shen{think-the-order: defend BGP path collection}
// Defense: the distributed verification is fundamentally collecting paths;
One may concern existing control-plane like BGP and OSPF already collected paths, and predicts can be directly verified on their paths. // the paths collected by BGP can be wrong since they can be buggy (with emerging of white-box switches, there are different versions of software constantly changing). 

\subsection{Distributed Verification Protocol}
\richard{DV is SIMPLE}

\shen{Given a requirement:} $\forall p \in hs_i, DP^A(p) \neq \emptyset, \mathcal{P}_c \subseteq DP^A(p) \subseteq \mathcal{P}_s$. A path-set $\mathcal{P}$ may be specified using multiple sets and set operations $\{\cap, \cup\}$.

\shen{clarify there is only a single DFA}
\begin{proposition}
The DFA for $\mathcal{P}_c$ forms a sub-graph of $\mathcal{P}_s$ (using subsets of states and transitions).
\end{proposition}

\shen{1. DFA} \shen{example showing super-source} Inspired by studies in network configuration synthesis~\cite{merlin, propane, contra}, \DistVeri constructs a deterministic finite automata (DFA) to compactly capture requirements and decompose it into sub-DFAs for every node. Each set specified using Regex can be compiled into a DFA. A DFA $M_k$ is defined as a 5-tuple $(\Sigma_k, S_k, F_k, s_{k}^0, \sigma_k)$. The alphabet $\Sigma$ consists of devices involved in requirement. $S_k$ is the set of states while $F_k \subseteq S_k$ are final states and $s_{k}^0$ is the initial state. Transition function $\sigma_k: S_k \times \Sigma_k \rightarrow S_k$ gives all the valid transitions while invalid transitions are omitted here.

Combining two set together is computing the product of their DFAs using standard approach. Consider two DFAs $M_1$ and $M_2$, the DFA for $M_1 \cap M_2$ us $M' = (\Sigma_1 \cup \Sigma_2, S_1 \times S_2, F_1 \times F_2, (s_{1}^0, s_{2}^0), \sigma')$ where $\forall a \in \Sigma', (s_1', s_2') \in \sigma'((s_1, s_2), a))$ if and only if $s_1' \in \sigma_1(s_1, a)$ and $s_2' \in \sigma_2(s_2, a)$. Given the definition of intersection $\cap$, the union $\cup$ is defined in the same way except the final states are $(F_1 \times S_2) \cup (S_1 \times F_2)$ instead of $F_1 \times F_2$.
%Contra combines sets using $\cup$ as preferrence; \DistVeri combines sets mostly using $\cap$ as requirement

\shen{semantics of DFA}: 
A requirement-compliant data-plane can be mapped to the global DFA. One can imagine a packet start from the initial state $s_0$, when it appears on the a source device $j$, it takes a transition from $s_0$ to $\sigma(s_0, j)$. Then each state $s$ with $s.node = j$ forwards packet according to $FIB_i^j$: when the FIB takes action to forward packet to a device $j$, this packet goes to $\sigma(s, j)$ in DFA. A state $s$ in DFA can be uniquely mapped to a device $j$, which is also the token transiting to $s$, notated as $s.node = j$. A single device may have multiple states and a packet will reach one of them depending the path it has traversed through.
% If there is no such transition, it means violation..

\shen{2. CDT} % // a nugget: CDT 
A naive verification approach (CDT) is centralized, which has access to the global DFA and the all FIBs. This approach helps understanding our key idea: for each state, computing the header space that will cause violation. For a state $s$, the violation can be divided into two types: (1) its FIB forwards packets incorrectly and (2) its FIBs forwards packets correctly but the downstream states has violation. 

For a state $s$, its first type of violation are stored in $s.H^0$ (shown in the code below). Specifically, a FIB can forward packets correctly if and only if it uses available physical links and follows the egress transitions for state $s$, \ie, the group of next-hops should be a subset of transitions in $\mathcal{P}_s$ and also a superset of transitions in $\mathcal{P}_c$; Otherwise, the header space of such entry will cause the first type of violation. 

\begin{itemize}
    \item strawman solution: collect all FIB entries to source; challenges: message overhead and computation overhead.
    \item C1. block (1): collect FIB entries that will cause violation
    \item C2. block (2): send violation entry to upstream to construct a path ending at  violation
    \item C3. aggregate entries for different violations into a single header space
    \item C4. distribute computation and also block message when the header space becomes empty
\end{itemize}

design principles / key ideas
oracle (insights, benefits)

=====

remaining question: how to construct oracle?
1. how to construct DFA
2. how to utilize DFA for

\begin{algorithm}[h]
    \SetAlgoLined
    \KwData{$N.VFIB$}
    \ForEach{$entry \in N.VFIB$} {
        $H^0 = \emptyset$\;
        \ForEach{$entry$} {
            \If{$entry$ not follow step-0 oracle (C1)}{
                $H^0 = H^0  + entry.match$\;
            }
        }
        Send $H^0$ to upstream neighbours following oracle (C2)\;
    }
\caption{Distributed Verification (DDT) Msg Initialization}
\end{algorithm}

\begin{algorithm}[H]
    \SetAlgoLined
    \KwData{FIB}
    \KwResult{Violation packet space for each state $\{s.H\} (C3)$}
    \ForEach{$s$} {
        $s.H^0 = \emptyset$\;
        \ForEach{$entry \in s.node.FIB$} {
            \If{$entry$ not follow step-0 oracle (C1)}{
                $s.H^0 = s.H^0  + entry.match$\;
            }
        }
    }
    \ForEach{$s$ in oracle order (C2)} {
        $s.H = s.H^0$\;
        \ForEach{$entry \in s.node.FIB$} {
            $s' = entry.action$\ oracle;\;
            $s.H = s.H + entry.match \wedge entry.reverse(s'.H)$\;
        }
    }
\caption{Centralized Verification (CDT)}
\end{algorithm}

% CDT: all H^{(1)} should be directly computed from H^{(0)}, then we get rid of intermediate states; It explains why we can do distributed async protocol
\begin{algorithm}[H]
    \SetAlgoLined
    \KwData{FIB}
    \KwResult{Violation packet space for each state $\{s.H\} (C3)$}
    \ForEach{$s \in DFA$} {
        $s.H^0 = \emptyset$\;
        \ForEach{$entry \in s.node.FIB$} {
            \If{$\sigma(s, entry.action)$ not follow $DFA$ and $link$-$state$ (C1)}{
                $s.H^0 = s.H^0  \cup entry.match$\;
            }
        }
    }
    \ForEach{$s \in DFA$ following reversed topological order (C2)} {
        $s.H = s.H^0$\;
        \ForEach{$entry \in s.node.FIB$} {
            $s' = \sigma(s, entry.action)$\;
            $s.H = s.H \cup (entry.match \wedge entry.reverse(s'.H))$\;
        }
    }
\caption{Centralized Verification (CDT)}
\end{algorithm}

For a state $s$, the second type of violations are recursively collected from its downstream states. This recursive process is terminable when the DFA is acyclic \shen{claim loop-free}. Taking the header space from downstream $s'$, the computation of header space was first proposed by ~\cite{kazemian2013real}: it utilizes reverse function of modification function to compute the header space for $s$.

% clarify the packet spaces from different src can be different and we take the intersections.
As a result, each source device has a header space capturing all packets that will cause violation. This header space is unique since each device $j$ has at most one source state ($\sigma(s_0, j)$) transiting from $s_0$. In general cases, a device can have different violation header space for each state.

\shen{3. DDT} \richard{DDT w/ example} \qiao{decompose DFA into local DFAs}

\begin{figure}[t]
\centering
\includegraphics[width=1\columnwidth]{images/dv-back-propagation.png}
\caption{\small{Illustratration of a back-propagation message}}
\label{fig:dv-back-propagation}
\reducespace
\end{figure}
\shen{local DFA and violation tables} A key observation of CDT is its data-structures and computations can be partitioned to devices in the whole network (as shown in Fig~\ref{fig:dv-ddt-mapping}). Consider a state $s$, its violation table and ingress/egress transitions are assigned to device $s.node$. And its computations can be done locally or based on the communication with its ingress and egress states.

This partition gives us the \DistVeri protocol which computes the same results with CDT. This protocol has 2 components: (1) local violation entry generation; and (2) back-propagation. The \textbf{local} part is the same as the first part of CDT except every device can run in parallel. 
% give intuition why: the data structure and computation in CDT can be partitioned nicely to the whole network.

\textbf{Back-propagation}: as shown in Fig~\ref{fig:dv-back-propagation}, when a state has updated the header space for its violation table, it back propagates this to ingress states $s_{in}$.  In real network, such message is actually sent to $s_{in}.node$. This process can be done incrementally like existing work~\cite{khurshid2013veriflow}, \ie, only announce the delta when header space changes. \shen{Particularly, a state in coverage-set doesn't need to back-propagate header space; Instead, it announce a short message to indicate whether there exists violation.} % clarify when the local violation has intersection with coverage-set, we can directly notify the source with this entry w/o computation; the src-V must be non-empty, but the precise packet-space is unknown due to packet-modification

\begin{proposition}
Back-propagation computes the same results even under out-of-order messages and link-failure. 
\end{proposition}
\textbf{Scratch of Proof}: Out-of-order messages are fine since they are  fundamentally collecting different violation paths. When link-failure, consider a requirement-complaint path-prefix, the first device, which forwards packets incorrectly or to a unavailable link, will locally detect violation and trigger back-propagation.

% // Incremental update: probably dummy local-recomputation algorithm (claim switch has sufficient computation resources)

% Composition: transient violation and we use  eventual consistency mode
% 
% Each CP can use MPLS to solve transient violations. 
% argument for complexity, each suffix of violation paths has (bidirectional) 1-to-1 mapping to entry in violation table.

\subsection{Extensions} 
\richard{Claim basic protocol and extensions}

\shen{MS'19 as a special caes}
Operator may wonder the real-world usage of $\mathcal{P}_c$, for example, Azure~\cite{jayaraman2019validating} requires $\mathcal{P}_c = \mathcal{P}_s$. This case degenerates back-propagation to local contract: when a state locally detects a violation, there must be a violation in global. \textbf{Proof of scratch}: there are only 2 cases: (1) a local violation can be triggered by an incoming packet; (2) there is no such incoming packet due to violations in the upstream.

\shen{clarify} The necessary and sufficient condition for a requirement with $\mathcal{P}_c = \mathcal{P}_s$ to be satisfiable: each device $j$ has a safe action which follows transitions of all states $s$ with $s.node = j$. \textbf{Proof of scratch}: otherwise, given a non-safe action, there must be a state causing violation when packets arrive it; and packets can always arrive it according to $\mathcal{P}_c$.

% consistency model for local safe action: an example on how multiple control plane composition can help improve MS local verification (e.g., switching from buggy OSPF-1 to correct OSPF-2 when OSPF-1 gives a wrong set of available NHs) 

\richard{conditional transition}
$\mathcal{P}_s$ may include backup-path that only can be used under link-failure. Such scenario can be supported by extending condition transition in DFA: for state $s$, the availability of a transition 
depends on the links connected to $s.node$. In particular, the transitions for backup-path is available 
only when the link for the primal-path is down.

\shen{Scalability: use shortest-path instead of loop-free;}
An interesting result is: the complexity of verification may increase or decrease when adding more requirements. The complexity actually depends on the number of states in DFA, which increases for 
way-pointing (stateful routing) and decrease for shortest-path (stateless routing).

\shen{scalabiity: abstract topo}

\shen{prefix used by coverage-set}
Given the global DFA and distributed verification protocol, an interesting observation is: path in $\mathcal{P}_c$ are not necessarily to be complete. They can be path-prefixes. The verification can guarantee those states in path-prefixes are available for all header space and does not require coverage for other states. Such path-prefixes are already supported by our path grammar and regular expressions: they are paths without end-sign ($\$$).



\subsection{Other Concerns (remove later)}
\shen{handle multi-src using super-src in a DFA}

\richard{move FB-requirements to eval-sec} % Reachability (with VIP), Shortest-path, Backup-path, Traffic-engineering 

//Handle more complex verification scenarios
group table
anycast (e.g., VIP)
multicast (less priority, but please handle)
multiple sources (e.g., multiple border routers for traffic entering a network)
	Add a supersource directly connected to multiple sources. Multiple sources need to synchronize on verification results.
integration of FSD and DFA: please try to merge them
adapter for each CP (default is just FIB), to extract additional FRR info
	Add a virtual link for each physical link in the topology, representing the link protection tunnel. // Pull FRR from CP to Carbide domain
Assume a single CP cp being used. At T0 link e1 fails. CP cp has FRR capability to handle this failure.
// TBD: 0. There is a pre-verified CP doesn’t use e1; Carbide immediately switch to it.
1. This FRR can; It is be pre-verified by DV using group table model (e.g., ECMP, EIGRP’s feasible backup path, BGP RIB). * emphasize not total blackbox *
We do not switch. Carbide does not introduce delay.
2. This FRR cannot but it has link protection, in which e1.head uses a tunnel (uses an outer header) to send traffic to e1.end. Defense: this is naturally captured by DV’s group table model. A tunnel can be specified as path-requirements for packets taking e1.head as source. Those paths are provided in group table but not necessarily to be used in most time. Path-requirements such as shortest-path and waypoint avoidance are not handled in tunnel. For tunnel, the only requirement is reachability. 
// Think-the-order: define the path-requirements (and probably specify user language) // clarify we allow generic requirements and path-requirements are special cases
// TBD: an alternative solution is to combine it with link-state verification and put as an additional low-layer verification.

\shen{CP-selection concern}
// CP-selection announcement TBD: this part is coupled with composition
When verification has been done, each source knows the violation of its downstream. For each packet space, a source will announce a set of CPs that can be used for its downstreams. A node should collect the announcement from all sources and computes the intersections. The most preferred one in the result will be the selected CP for a packet space. // prove the selection is consistent // clarify the packet spaces from different src can be different and we take the intersections.

// TBD: Given a source cannot figure out when the verification has been done, it may periodically compute the set of CPs

==> backup.tex <==





\section{Backup notes}
\subsection{overview-dv non-wordy version}
\para{\DistVeri{}: a novel, light-weight distributed verification tool (Section~\ref{sec:dv})}.
\qiao{tool, protocol, or framework?}
%The goal of the distributed verification protocol 
A fundamental challenge of composing control planes is to check in real time
whether the paths constructed by the current network data plane satisfies certain requirements. Previous
data plane verification tools~\cite{kazemian2012header,
khurshid2013veriflow, kazemian2013real, yang2015real, horn2017delta} adopt a centralized
design: a logically centralized server is deployed to collect and analyze the
whole data plane of the network. This design has high communication and
computation overhead, and has a single point of failure at the centralized
server. As such, it does not suit the need for control plane composition.
(\qiao{weak argument..., refine later})

In contrast, \system{} designs a novel, light-weight distributed verification
tool called \DistVeri{} to achieve real-time data plane verification. The basic
insight of \DistVeri{} is: \textit{by leveraging the knowledge on the network,
\ie, topology and requirement, one global verification task can be decomposed
into multiple local tasks that can run on network devices individually.} In
particular, to verify a global requirement, each device individually checks its
data plane (\eg, forwarding information base and access control list) to
identify all the local violations of the requirement, and recursively collects
all the violations at the data planes of downstream devices. In the end, the
ingress devices, where packets enter the network, have the complete knowledge on
all the violations of the requirement in the data plane of the whole network.

\DistVeri{} is a generic data plane verification tool that can verify a wide
range of common requirements (\eg, reachability, waypoint, loop-free and
fault-tolerance) under different forwarding scenarios (\eg, unicast, anycast,
multicast, and load-balancing). When the requirement and network topology
satisfy certain conditions (\qiao{specify it}), \DistVeri{} degenerates from
distributed verification to pure local verification, making the local validation
design~\cite{jayaraman2019validating} become its special case.

%(2) \DistVeri{} can be integrated with the centralized design
%(\qiao{this is a little confusing...}) to
%verify more complex requirements (\eg, route symmetry and disjoint-path).

\para{\textit{CPComposer} a novel control plane composition framework}. 
In order to compose multiple control planes, each device runs an online CP
composer which takes as input the verification results and dynamically composes
the forwarding rules from multiple vFIBs to compute a unified physical FIB
(pFIB) to enforce at the data plane. An important benefit of \system running
multiple CPs is that maybe one CP cannot satisfy all the requirements, but
\system allows different packets to use different CPs. 

\system adopts a flexible composition model that allows users to specify the
control plane usage and preference for each packet space. Based on the
verification results, the source of each packet can compute and select the most
preferred CP that is verified to process the packet. To further improve
reliability and to quickly response to failures,  any nodes other than the
sources are allowed to dynamically switch among CPs while ensuring the
correctness requirement to be satisfied. Another novel piece in the composer is
to include the fast reroute (FRR) ability of each control plane. Specifically,
the backup paths (or tunnels) are verified at background, in advance of network
failures, therefore upon network events, the composer can make the most
responsive action to recover traffic, by either using the current control plane
FRR or switching to another control plane that is verified.




\subsection{overview-dv wordy version}
\para{\DistVeri{}: a novel, light-weight distributed verification tool (Section~\ref{sec:dv})}.
\qiao{tool, protocol, or framework?}
%The goal of the distributed verification protocol 
A fundamental challenge of composing control planes is to check in real time
whether the paths constructed by the current network data plane satisfies certain requirements. Previous
data plane verification tools~\cite{kazemian2012header,
khurshid2013veriflow, kazemian2013real, yang2015real, horn2017delta} adopt a centralized
design: a logically centralized server is deployed to collect and analyze the
whole data plane of the network. This design has high communication and
computation overhead, and has a single point of failure at the centralized
server. As such, it does not suit the need for control plane composition.
(\qiao{weak argument..., refine later})

In contrast, \system{} designs a novel, light-weight distributed verification
tool called \DistVeri{} to achieve real-time data plane verification. The basic
insight of \DistVeri{} is: \textit{by leveraging the pre-knowledge on
network, \ie, topology and requirement, one global verification task can be
decomposed into multiple local tasks that can run on network devices
individually.} Given a device, its local task only requires its own data plane
and the local task results of some of its neighbors as input. As such, a global
verification task can be accomplished by devices computing their local tasks and
propagating the results recursively.



Specifically, given a user-specified requirement, \DistVeri{} verifies the
validity of the current data plane with three key steps: (1) transform the
requirement and the network topology into a deterministic finite automata (DFA)
that represents all requirement-compliant paths in the network; (2) each device
locally compares its data plane (\eg, forwarding information base and access
control list) with the state transition in the DFA to identify all the %possible
violations of the requirement at its data plane; and (3) each device recursively
collects all the violations at the data planes of devices corresponding to the
downstream nodes in the DFA. In the end, the ingress devices, where packets
enter the network, have the complete knowledge on all the violations of the
requirement in the data plane of the whole network.

\DistVeri{} is a generic data plane verification tool that can verify
a wide range of typical requirements (\eg, reachability, waypoint, loop-free and
fault-tolerance) on different forwarding actions (\eg, unicast, anycast,
multicast, and load-balancing). It is also shown in later part of the paper that
(1) when the requirement and network topology satisfy certain conditions
(\qiao{specify it}), \DistVeri{} can degenerate from distributed verification to
pure local verification, making the local validation design in~\cite{jayaraman2019validating} a special case
of \DistVeri{}; (2) \DistVeri{} can be integrated with the centralized design
(\qiao{this is a little confusing...}) to
verify more complex requirements (\eg, route symmetry and disjoint-path).


\subsection{random notes}
Specifically, \DistVeri{} allows an operator to specify a requirement
on network's data plane (\eg, reachability, waypoint routing and ECMP) as a
tuple of a packet space and a sequence of logical expressions on paths.
\qiao{depending on the grammar... to update later.} It transforms this
tuple and the network topology into a deterministic finite automata (DFA) that
represents all requirement-compliant paths in the network. In this way, the
problem of data plane verification is reduced to checking whether there exists a
path that is constructed by the current data plane and not accepted by the DFA.

Next, \DistVeri{} leverages this reduction to decompose a global verification task into local
tasks run individually on network devices. In particular, given a network
device, \DistVeri{} augments its forwarding information base to also match on
ingress state of the DFA, 


DFA defines all valid state transition, expand FIB to also match on ingress
states in DFA, 

DFA as a compact representation of all requirement-compliant paths. 
State-FIB: Expands its FIB to also match on states in DFA. 
False-FIB: Entries in State-FIB that forward to requirement-noncompliant next-hops.
Back Propagation: Each node recursively collects False-FIBs from its downstream nodes in the DFA to compute all the entries in its State-FIB that forward to requirement-noncompliant downstream paths.




extracts its data plane (\eg, the forwarding information
base and access control list) as a match-action table.
%, where the  match-fields and depend on the application specific integrated circuit
%(ASIC) of the device. 
A group-action semantic is used to model load-balancing, fault-tolerance,
multicast and anycast, (\qiao{how to handle packet transformation?}). 
\DistVeri{} then augments this table by (1) adding a new match field matching the
ingress state of the DFA and ..

Just say augment the FIB, each device check argumented-FIB violation at immediate
nexthop, and recursively propagate.

DV protocol

MS as a special case.

Extending DV protocol to more generic requirements. 


the protocol introduces a group table abstraction of forwarding
information base. 


The distributed verification protocol
is a generic service that checks the validity of the datapath
in the network. 




==> composition-framework.tex <==
\section{Composition Framework}
% Introduce (predicate, CP) tuple based composition framework here.

\input{Composition/wrtie-up}

==> dv-grammar.tex <==
\vspace{-2mm}
\subsection{Verification Requirements Specification}\label{sec:dv-grammar}
A wide range of common, important verification requirements (\eg, reachability, waypoint, loop freeness and fault tolerance) can be expressed as a set comparison expression between the  single-forwarding path set constructed by $\{FIB_i^j\}_j$ and a topology path set defined by predicates of regular expressions (Figure~\ref{fig:dv-grammar}). 

\DistVeri designs a simple distributed verification algorithm in the next subsection to verify these requirements, efficiently.

\para{A running example}. 
Take the network in Figure~\ref{fig:dv-example-topology} as a
running example. $S$, $A$ and so on are the identifier labels of network devices.  
%\shen{refer to multiple hosts using a label}
$S$ and $D$ each has an IP label 10.0.1.0/24 and 10.0.2.0/24, respectively,
denoting to the subnet each one is connected to.
The following program specifies that the operator wants to verify whether the
traffic from source IP 10.0.1.0/24 to destination IP 10.0.2.0/24 is always
delivered (\ie, reachability) after passing $W$ (\ie, waypoint), without any
loop (\ie, loop-free).



%\DistVeri provides a simplified grammar  that can specify , and 
 
%\shen{This algorithm is 
%more efficient since it processes each path in isolation. As a contrast, a generic 
%verification involves the exponential complexity of path-combinations.} 
%This discussion 
%presents a simplified verification specification grammar that 5%allows operators to 
%specify these requirements. 

% An operator can use this simplified grammar to specify a verification requirement
% as a tuple of (1) packet space $h$ defined by predicates on packet headers, and
% (2) a set comparison expression between the single-forwarding path set
% constructed by $\{FIB_i^j\}_j$ and a topology path set defined by predicates of regular expressions. 

\begin{figure}
\ttfamily
\footnotesize
\begin{tabular}{r L  l}
       h & \in & packet headers
    \\ f & \in & header fields
    \\ v & \in & header field values
    \\ label & \in & device labels 
    \\ pkt\_predicate & := &  (h.f=v)
    \\ & | & (pkt\_predicate [$|$, \&] pkt\_predicate)
    \\ & | & !pkt\_predicate
%    \\ path & := & $\&$ $|$ $\$$ % a sequence of devices, but
%    \\ & | & [label] path % also considered as a set of devices
\\    topo\_path\_set & := & $P_i^{any}$
%    \\
	\\ regex & := & ...
%\\
    \\ path\_set & := & regex
%& $DP^A(p)$
%    \\ & | & $DP^M(p)$
    \\ & | & (path\_set [$\wedge$, $\vee$] path\_set)
%	\\
	\\ps\_compare & := & topo\_path\_set [$\subset, \supset, =, $] path\_set
    \\ & | & ps\_compare [$\wedge$, $\vee$] ps\_compare
 %   \\
%    \\ requirements & := & $\forall$ p $\in$ pkt\_spec, path\_set [$\subset, \supset, =, \neq$] path\_set
%    \\ consistency & := & per-packet | relaxed | ...
    \\ requirement & := & pkt\_predicate $\rightarrow$ ps\_compare
  %  \\
\end{tabular}
%\normalfont
	\caption{\small{A simplified grammar of \DistVeri \ReqLang.}}\label{fig:dv-grammar}
\reducespace
\end{figure}


%, and a consistency requirement during data plane update (details in Section~\ref{sec:consistency}).  

%\para{Example}. 

\begin{figure}
{\footnotesize
\begin{verbatim}
h: {src_ip = 10.0.1.0/24 | dst_ip = 10.0.2.0/24};
reachability: {[10.0.1.0/24].*[10.0.1.0/24]$};
waypoint: {.*W.*$};
loopfree: 
    foreach n in V: 
        loopfree &= {[^n]*$)|([^n]*)n([^n]*)$)};
topo_pathset: reachability & waypoint & loopfree;
h->dp_path_set.issubset(topo_pathset); 
\end{verbatim}
}
\caption{\small The operator specifies reachability, waypoint and loopfree
	requirements.\qiao{Shenshen: help add line number.}}
\label{fig:dv-example-requirement}
\end{figure}

Specifically, the program first defines a packet space $h$ to be the set of
packets with source IP 10.0.1.0/24 and destination IP 10.0.2.0/24. 
Next, it uses regular expressions to
define the set of paths in the network that satisfy the reachability, waypoint
and loop-free requirements, respectively. At the end, the verification
requirement is expressed that the single-forwarding path set generated by the data plane of
the network for packet space $h$ must be a subset of the path set in the
topology that satisfy all three requirements.
%\shen{maybe try to introduce coverage-set...}

%The remaining of this section presents a novel, efficient distributed verification algorithm to efficiently
%verify the requirements specified by the simplified grammar. 
%The verification algorithm for the complete grammar is presented in . 

%\qiao{shortest path as an extension, MS as a special case as an extension, path
%prefix as an extension. They are not mentioned here.}








%\DistVeri provides a novel, efficient algorithm based on deterministic finite
%automata (DFA) traversal, which allows each device to locally verify its own FIB, 
%and recursively collect the results of downstream devices. Specifically, \DistVeri gives the following
%sufficient condition on the applicability of this DFA-based verification
%algorithm:

%\begin{proposition}[Applicability of the DFA-based verification algorithm] \label{prop:dfa-applicability}
%Given a requirement $r$ on packet space $h$, if it can be expressed as a logical
%	expression on path set $P_r$ and path set $P_i(h)$ that only uses
%	$\subset$ and logical operators, it can be verified by the DFA-based
%	algorithm.
%\end{proposition}

==> evaluation.tex <==
\section{Evaluation}\label{sec:evaluation}

% This section illustrates the benefits of \system, evaluates its overhead under different network settings and demonstrates how it can handle large-scale network verification.
% % The set of experiments we conduct aim to answer the following questions: a) what are the benefits of Carbide? b) what kind of network properties Carbide can verify, \ie, what is the effectiveness of Carbide? c) how Carbide scales to large networks, in particular, can Carbide work on data center scale networks? d) what is the overhead of running Carbide on a network device?



% \begin{table}[t]
% \setlength{\abovecaptionskip}{0.1cm}
% \setlength{\belowcaptionskip}{-0.cm}
% \centering
% \footnotesize
%     \begin{tabular}{|c|c|c|c|}
%     \hline
%     Network & Type & \# nodes & \# links \\
%     \hline
%     Abilene & Backbone & 11 & 14\\
%     \hline
%     AT\&T & Backbone & 25 & 56\\
%     \hline 
%     Rocketfuel (AS 1755) & Backbone & 172 & 381 \\
%     \hline 
%     Facebook & Data center & x & x \\ 
%     \hline
%     \end{tabular}
%     \caption{\small{Summary of network topologies we used.}}
%     \label{tab:topologies}
%     \reducespace
% \end{table}

% \subsection{Methodology}
% We evaluate \system in a variety of backbone networks described in Table~\ref{tab:topologies} using Docker~\cite{docker} based implementation of \impl. We model each switch as a separate container where it can run Quagga~\cite{quagga} Routing Suite as CPs (providing BGP and OSPF) and OpenFlow-based SDN. \kerim{this is only correct for link failure experiment, should we state here? We further deploy two real Openflow white-box switches to validate the feasibility. Their models are Pica8 P-5401 and Dell Z9100-ON.} We further analyze the scalability of \system using large scale data center topologies shown in Table~\ref{tab:topologies}.


% % \begin{figure}
% % \centering
% % \setlength{\abovecaptionskip}{0.1cm}
% % \setlength{\belowcaptionskip}{-0.cm}
% % \includegraphics[width=0.6\columnwidth]{images/platform.png}\caption{\small{The Architecture of Emulation/Simulation Platform(s)\kerim{Either a single figure or two subfigures}}}\label{fig:platform}
% % %\reducespace
% % %\vspace{-1.5em}
% % \end{figure}

% % \begin{figure}
% % \centering
% % \setlength{\abovecaptionskip}{0.1cm}
% % \setlength{\belowcaptionskip}{-0.cm}
% % \includegraphics[width=0.6\columnwidth]{images/topology.png}\caption{\small{\kerim{Two subfigures showing a) k-ary data center topology b) "real" topology (from TopologyZoo)}}}\label{fig:topology}
% % %\reducespace
% % %\vspace{-1.5em}
% % \end{figure}


% \begin{figure}[t]
% \setlength{\abovecaptionskip}{0.1cm}
% \setlength{\belowcaptionskip}{-0.cm}
% \begin{tabular}{@{}c@{}c@{\hspace{1em}}c@{}c@{}}
% \centering
% \includegraphics[width=0.50\linewidth]{images/coldstart_buggy.png} &
% \includegraphics[width=0.50\linewidth]{images/coldstart_nonbuggy.png} \\
% \small(a) & \small(b)
% \end{tabular}
% \caption{\small{Convergence times in continuous deployment experiments with a single control plane (SCP) and centralized verification (CV). (a) The newly deployed CP is buggy and global rollback to the previous version is performed. (b) The newly deployed CP is not buggy but there are transient violations due to mixed rules from the old and new CPs.}}\label{fig:coldstart}
% \reducespace
% \vspace{-1em}
% \end{figure}

% \subsection{Switch Software Continuous Deployment}\label{ssec:coldstart}
% The goal of this set of experiments is to evaluate the benefits \system compared to single control plane (SCP) with centralized verification (CV) deployment.

% \para{Methodology.} In this experiment, we deploy \impl on the AT\&T backbone topology shown in Table~\ref{tab:topologies}, and pick OSPF as the control plane and used NetPlumber~\cite{} based centralized verification. We assume that the network is running a stable version of OSPF (denoted $CP_1$) and the data plane is fully deployed and verified. At time $t_0$, we deploy a new version of OSPF binary on each switch, namely $CP_2$. We assume that the data plane only changes when there is new rule update, \eg at $t_0$ the data plane contains the rules generated by $CP_1$. We then incrementally verify each FIB update by $CP_2$ pushed to the data plane via CV. \kerim{Single sentence about requirement, current requirement is shortest path} We consider two cases for $CP_2$ deployment shown in Figure~\ref{fig:coldstart}. We first use a buggy version of OSPF that generates non-shortest paths for some destinations shown in Figure~\ref{fig:coldstart}(a). ... Secondly, we deploy an OSPF without any bugs shown in Figure~\ref{fig:coldstart}(b). 


% We start with a simple experiment to illustrate the benefits of \system, compared with a traditional single CP, centralized verification (SCP+CV) setting. In this experiment, for both \system and SCP+CV an initial CP (CP1) is fully deployed and verified. At time T0, a new CP (CP2), which is a new binary, needs to be deployed. For SCP+CV, the new binary starts at each switch at T0. \calvin{Old FIB entries of CP1 will still be valid until being overwritten by CP2.} Whenever each switch updates a rule in its FIB, the update will be immediately sent to the CV server to detect errors, realizing efficient incremental verification. \calvin{Here comes the complex design issue of SCP+CV: during the initialization process of CP2, parts of the FIB entries is installed CP1 and others by CP2. Mixing new and old entries server may detect some transient violations, but it is difficult ,if not impossible, for it to determine whether this violation is temporary or is inherent in CP2. }
% \para{Results.} Figure~\ref{fig:coldstart} . \system, however, has zero policy-incompliant time in both scenarios since 
% %  As soon as the CV detects an error, it asks all switches to rollback to CP1 by killing the CP2 process and restarting the CP1 process at each switch.
%  Figure X(a) shows the results. At time T1c, the edge switch sw1 installs a new rule computed by CP2 which sends traffic to dst to sw2, forming a loop. This erroneous FIB entry is sent to the CV server, which detects the error and asks each switch to restart CP1. Since the initial convergence time is slow, it takes until T2c when the network re-converges. It is indeed possible to design an algorithm to not simply rollback to CP1. In such a case, the CV server then will need to become a global controller to coordinate the route replacement process across the whole network. Assume that care is not taken (\eg, using fixed static route), an FIB can cause the routes between the CV server and a switch to be disconnected, leading to a serious problem in such a centralized control scheme. \\
% % We conduct the same experiment using \system, and Figure X(b) shows the results. Also at T1c, the edge switch sw1 installs the wrong FIB entry into CP2. However, \system at sw1 immediately detects that the violation and starts the process to report the violation back toward the source. No routing loop is ever formed. At the same time, the correct routes from CP2 (\ie, not to dst) are still installed, replacing those from CP1.

% % In this set of experiments, we demonstrate how \system supports a popular switch software development principle \textit{deploy-early-and-iterate}. [FBOSS] \\
% % Suppose a stable control plane CPv1 is running in our network, and a new version CPv2 is being deployed to replace it. However, the rapid pace of evolving leaves the correctness and robustness of the control plane in question. Here we compare two approaches to guard against undesirable control plane behaviors, \system and centralized verification. \\

% % For centralized verification, we deploy a state-of-the-art real-time verification tool, NetPlumber[] in the central controller. The controller will collect all forwarding table entries from switches, apply verification and trigger rollback if CPv2 still has violation after convergence (foot note of convergence definition: We define convergence by no FIB update within xxx). With \system, we can coordinate both versions simultaneously and verify correctness in a distributed manner. \\
% % \para{Valid New Control Plane} We first consider the case where CPv2 is valid and complies with all requirements after convergence. Figure X shows that verification finishing time is almost the same for \system and centralized controller, but \system can flexibly mix CPv1 and CPv2 when CPv2 is initializing and thus reduce network downtime due to the update deployment. \\

% % \para{Invalid New Control Plane} Even though downtime caused by update can be eased by hot update techniques[citations], there is no way for (SCP+CV) to confirm the violation before CP convergence. We will repeat the above experiment with a misconfigured CPv2, demonstrating what kind of risk (SCP+CV) will cause and how \system can prevent it. \\
% % From figure Y, we can see that in (SCP+CV) approach, packets will be forwarded using policy-violating path until the violation gets confirmed and starts rollback. Meanwhile, for /system, source node will always choose valid CP based on real-time violation table. Thus, the violating path generated by CPv2 will never be chosen (be more careful about this statement, need to coordinate with consistency model in previous sections). \\
% \calvin{Use new figure to demonstrate this part. Show how violation portion of (SCP+CS) scheme will change under three cases (1.Valid new CP deployed correctly; 2.Invalid new CP trigger rollback; 3.Valid new CP but trigger rollback due to false positive.}

% \subsection{Failure Recovery}
% \vspace{-0.5em}
% \begin{figure}[t]
% \setlength{\abovecaptionskip}{0.1cm}
% \setlength{\belowcaptionskip}{-0.cm}
% \begin{tabular}{@{}c@{}c@{\hspace{1em}}c@{}c@{}}
% \centering
% \includegraphics[width=0.5\linewidth]{images/sdn-ospf-sdn.png} &
% \includegraphics[width=0.5\linewidth]{images/sdn-ospf1-sdn.png} \\
% \small(a) & \small(b)
% \end{tabular}
% \caption{\small{Packet receiving rate for the fast recovery experiments. The failure in (a) affects both the SDN and OSPF CPs, while that in (b) affects only the current SDN. }}\label{fig:sdn-ospf1-sdn}
% \reducespace
% %\vspace{-1em}
% \end{figure}

% \calvin{We need to state clearly about local switching behavior, avoid conflicts with Composition section}\\

% The goal of this set of experiments consists in evaluating the effectiveness of \system in recovering from link failures. 

% \para{Methodology.} We randomly
% select a pair of nodes (\eg router 313 to router 230) and generate UDP traffic between them by running iperf~\cite{iperf} at a rate of 100Mbps.
% For the SDN CPs, we implement the algorithm in BwE~\cite{kumar2015bwe} to compute the paths.
% We then randomly select links to fail on one of the paths used by the UDP traffic.
% For the SDN CPs to recover from the failures, we implement a reactive approach. That is, when a failure happens, the device that detects it sends a control message to the controller to recalculate alternative forwarding paths and update the vFIB of the affected devices accordingly~\cite{sharma2012demonstration}. 
% \kerim{Identify \system setting: local switching and eventual consistency model}
% For each run, we measure the downtime defined as the amount of time between the moment the destination stops receiving packets because of the  failure to the moment the receiver starts receiving packets again. We repeat this process for 10 runs.

% \para{Results.} 
% Figure~\ref{fig:sdn-ospf1-sdn} illustrates some of the patterns we  observed: First, in Figure~\ref{fig:sdn-ospf1-sdn}(a), the failure affected both SDN and OSPF CPs. In other words, both CPs used the failed link for the next hop. As such, at $t_1$, no valid route can be used, leading to a throughput of 0. Then, after OSPF discovers an alternate path, \system uses OSPF to forward traffic, and the throughput starts increasing at $t_2$. Finally, after the SDN recovers the route, the device uses the OpenFlow rules to forward traffic, and the rate increases further starting from $t_3$. In Figure~\ref{fig:sdn-ospf1-sdn}(b), the link failure affects only the SDN CP. The device can immediately switch to OSPF to continue forward the packets. 


% Table~\ref{tab:table-downtime} summarizes the average downtimes of the two CPs, and that of \system{} across the runs.
% While the average downtime of the SDN CP is 112.861ms, the average downtime of OSPF is 22.572ms, and that of \system is even lower than both of them with 8.492ms.
% The results show that \system can reduce the downtime of SDN by more than an order of magnitude, and that of OSPF by 43\%. \kerim{if eventual consistency and local switching is used}
% While one may be surprised that on average, \system{} can recover faster than OSPF, the main reason is that in some runs, the SDN CP recovers faster, whereas in other runs, the OSPF CP recovers faster; and in every case, \system switches to the one that recovers the fastest.

% \begin{table}[t]
% \setlength{\abovecaptionskip}{0.1cm}
% \setlength{\belowcaptionskip}{-0.cm}
% \centering
% \footnotesize
%     \begin{tabular}{|c|c|c|c|}
%     \hline
%     ~ & SDN & \system & OSPF \\
%     \hline
%     Average downtime & 112.861ms & 8.492ms & 22.572ms \\
%     \hline
%     \end{tabular}
%     \caption{\small{Average downtime of using different systems.}}
%     \label{tab:table-downtime}
%     \reducespace
% \end{table}

\vspace{-1em}
% \subsection{Enforcing Network Requirements}
% \vspace{-0.5em}

% The goal of this set of experiments is to evaluate the effectiveness of \system in ensuring correctness requirements. 

% \para{Methodology.}
% We assume that the administrator wants to enforce waypoint routing. Specifically, all traffic to a specific destination (router 205) must traverse a firewall (at router 200). For the SDN CP to generate paths that are compliant with such requirement, we implement the algorithm in~\cite{ludwig2014good}.
% We then gradually fail random links in the middle of the topology, until a subset of nodes get partitioned and lose connectivity with the SDN controller. We focus on nodes in that partition, and considering the paths from every node in that partition to the destination router 205, we compare the fraction of paths that can traverse the firewall at router 200 and still complies with the requirement.
% For the SDN CP, although the controller is no longer reachable, packets are forwarded along the existing rules.
% For OSPF, this CP cannot enforce waypoint routing. Instead, when the computed path from a source to the target destination traverses the desired waypoint, the path is considered to satisfy the requirement. In contrast, when the computed path from a source to the target destination does not traverse the desired waypoint, the path is considered to violate correctness.
% Finally, with \system, given a source, if the path provided by the SDN CP satisfies the correctness requirement (\ie traverses the waypoint), the path is selected. Else,  if the path provided by the OSPF CP satisfies the correctness requirement (\ie traverses the waypoint), \system selects that path. Otherwise, the packets are dropped.


% \para{Results.} Table~\ref{tab:table-partition} shows the fraction of paths that satisfy the requirement. Before the network partition, the network consists of 171 source nodes. Using SDN, all of the paths satisfy the requirement. Similarly, with \system{}, the requirement is satisfied for all paths. In contrast, with OSPF, only 61\% of paths to destination 205 traverse the waypoint at router 200.

% After network partition, the component disconnected from the SDN controller consists of 122 nodes. \calvin{94\% of the paths continue satisfying reachability and waypointing (through a firewall) requirements--as opposed to 59\% for an Openflow SDN CP and 56\% for a vanilla-OSPF CP.} Using SDN, only 59\% of the paths satisfy the requirement. This is because the OpenFlow rules may be obsolete, and may forward packets along invalid paths and into blackholes. 
% Using OSPF, the fraction of paths that satisfy the requirement drops to 56\%, and the remaining 44\% would still allow packets to reach destination 205 but without traversing the waypoint 200, and would thus violate correctness. 
% In contrast, with \system, 94\% of the paths satisfy the requirement, and for the remaining 6\%, their traffic would be dropped. As such, \system guarantees correctness for all the paths.
% In summary, both \system and the SDN CP guarantee correctness whereas the OSPF CP may violate it. And, between \system and SDN, \system allows a larger number of paths to satisfy the requirement given that it can also use the paths not only from the SDN CP but also from other CPs when they satisfy the requirements. 
% \begin{table}[t]
% \setlength{\abovecaptionskip}{0.1cm}
% \setlength{\belowcaptionskip}{-0.cm}
% \centering
% \footnotesize
%     \begin{tabular}{|c|c|c|c|}
%     \hline
%     ~ & SDN & \system & OSPF \\
%     \hline
%     Before partition & 171/171 (100\%) & 171/171 (100\%) & 105/171 (61\%)\\
%     \hline
%     After partition & 72/122 (59\%) & 115/122 (94\%)& 69/122 (56\%)\\
%     \hline
%     \end{tabular}
%     \caption{\small{Fraction of paths that can reach router 205 after traversing waypoint at router 200.}}
%     \label{tab:table-partition}
%     \reducespace
%     \vspace{-2em}
% \end{table}

\subsection{Overhead and Scaling}
A concern of \system is its overhead. The overhead determines the cost and the scaling ability of \system. Compared with a traditional network with a single CP and no distributed verification, \system has the following overhead: (1) the overhead of running each additional CP at each switch; and (2) the overhead of \system messaging and processing to verify and compose CPs. Below we evaluate both. \\


\para{Control Plane Overhead}
\kerim{Addressing overhead of MCP. "do not provide sufficient confidence in whether this technique will work in practice on resource-constrained routers" and "I think an evaluation of overheads should appear. How many control planes can run in parallel. The authors keep drawing examples with 3 CP. How high this number can be? What would be the right number of CPs to have?"}
This set of experiments aims to demonstrate \system's feasibility by evaluating the overhead of running additional CPs in each switch. 
% \system compared to using a single control plane. We consider computation, memory and network resources on each network device, and evaluate how CPs and \system's distributed verification uses these resources in different scenarios.

\begin{figure}[t]
\setlength{\abovecaptionskip}{0.1cm}
\setlength{\belowcaptionskip}{-0.cm}
\begin{tabular}{@{}c@{}c@{\hspace{1em}}c@{}c@{}}
\centering
\includegraphics[width=0.48\linewidth]{images/verification_cpu_usage.png} &
\includegraphics[width=0.52\linewidth]{images/verification_memory_usage.png} \\
\small(a) & \small(b)
\end{tabular}
\caption{\small{Overhead evaluation of \system on a single CPU core device. (a) The average CPU usage and (b) the average memory usage in response to a real-time update. \kerim{Replace figure with k-CPs}}}\label{fig:overhead}
\reducespace
\vspace{-1em}
\end{figure}

\para{Overhead evaluation.} One may concern \system has considerable overhead compared with traditional single control plane architecture as it introduces extra computation in verification.
Figure~\ref{fig:overhead} shows the average CPU and memory usage of \system on a \emph{device with only a single CPU core} for a real-time update affecting an average of 30 LECs. In this experiment, we randomly trigger an update (\ie a link failure) in the network and measure the CPU and memory usage of different containers with 10 ms intervals for 3.5 seconds. Figure~\ref{fig:overhead}(a) shows that the CPU usage only peaks to 70\% for very short time when running Quagga computation, \system verification and composition, and at the rest of the computation it uses less than 40\% of CPU. We also see that \system almost uses no CPU when there is no update, except for some periodic updates (\eg Redis daemon updates). Figure~\ref{fig:overhead}(b) shows the memory usage for the same experiment, where LEC updates require less than 1 MB of memory. The 45 MB of memory is used for holding the state of \DistVeri (\eg verified LECs).

\kerim{Damping and resource allocation?}

\para{Methodology}
To understand the overhead of \system, we run three control planes (SDN, BGP, and OSPF) in our evaluation platform with different topology sizes. \kerim{exact specification of devices CPU/memory/link speed}. To understand the exact impact of \system on the network devices, we do not run any workload; then, we measure the CPU, memory and network usage of each device with 5 seconds pulling time. We particularly monitor each control plane instance, Quagga's Zebra daemon, and \system's agent for distributed verification and CP composition. We deploy Telegraf 1.10.2 in each node for monitoring where each Telegraf instance reports its stats to a centralized time-series database (Prometheus 2.15.2) instance. Specifically, we monitor the devices when the network is idle \ie, when there are no events in the network, when network updates moderately (\kerim{avg. event/sec}), and when the network is highly dynamic  (\kerim{avg. event/sec}). We run each experiment for an hour.

\para{Results}
Figure~\ref{fig:overhead}
\kerim{Expectation: Memory and network overhead is negligible for all cases, CPU is negligible when network is idle, CPU might be bursty when network is dynamic, especially because of DV, composition layer and Zebra}
From the results we can see, the lightweight verification and composition in \system is of limited overhead even on a large topology. Updating the LEC table often consumes the most of resources, but only a few of the LECs are updated for a single device thanks to the natural distributed computation framework.
In this experiment, we only consider reachability requirement though, and if more complicated requirements are considered, the overhead may increase, but is still reasonable under the computation power on commodity networking devices (\eg routers and switches).
Note that the results also include the overhead from multiple CPs, but the CP overhead is typically small compared with verification overhead, and it can be well limited by the stability control mechanism in \system as described in Section~\ref{ssec:stability}.

\\
\para{Verification and Composition Overhead} When \system is deployed and conducting real-time verification, it needs network bandwidth for propagating violation tables and CPU resources for processing those information. Here we randomly generate topologies of backbone networks with various sizes and measure the overhead after link up or link down event. \\
\calvin{Need more details for Dennis' settings and result interpretation.}
\begin{figure}
\centering
\setlength{\abovecaptionskip}{0.1cm}
\setlength{\belowcaptionskip}{-0.cm}
\includegraphics[width=0.6\columnwidth]{images/backbone_msg.pdf}\caption{\small{Amount of message sent by \system after one link event }}\label{fig:bb_msg}
%\reducespace
%\vspace{-1.5em}
\end{figure}

\begin{figure}
\centering
\setlength{\abovecaptionskip}{0.1cm}
\setlength{\belowcaptionskip}{-0.cm}
\includegraphics[width=0.6\columnwidth]{images/backbone_time.pdf}\caption{\small{Processing time of \system after one link event }}\label{fig:bb_msg}
%\reducespace
%\vspace{-1.5em}
\end{figure}

\\
\para{Scalability for Data Center Networks} As mentioned in previous sections, \system is capable to perform distributed verification for large-scale data centers, given particular requirements like shortest path. \calvin{In current organization, will data center mentioned in previous sections as a special case?} We first conduct a set of simulations on general fat tree topology to see how DFA size, memory usage and control message bandwidth grow with the network scale. \\
\para{DFA size} \calvin{Claim DFA size is linear with total switch amount} \\
\para{Message bandwidth} First consider only one switch has a forwarding entry going against the requirement. It will propagate this violation entry along the path to all the sources. Average bandwidth on each link is O(1/k) for single violation.
\calvin{Assume destination-based routing}

\begin{figure}
\centering
\setlength{\abovecaptionskip}{0.1cm}
\setlength{\belowcaptionskip}{-0.cm}
\includegraphics[width=0.6\columnwidth]{images/datacenter_msg_single.png}\caption{\small{Message sent by \system for a single violation FIB }}\label{fig:bb_msg}
%\reducespace
%\vspace{-1.5em}
\end{figure}

Then we consider more complex situations that involve burst errors in multiple devices. It will not grow linearly along the number of violation, especially when the number of violations becomes large enough to make propagation upstream paths overlap with each other. \calvin{Average, max, 50 percentile} \\
\begin{figure}
\centering
\setlength{\abovecaptionskip}{0.1cm}
\setlength{\belowcaptionskip}{-0.cm}
\includegraphics[width=0.6\columnwidth]{images/datacenter_msg1.png}\caption{\small{Message sent by \system for multiple violations caused by same error}}\label{fig:bb_msg}
%\reducespace
%\vspace{-1.5em}
\end{figure}

\para{Facebook real-world use case} As a key test on the scalability of \system, we apply it to a real, tier-one network, consisting of real topology and real requirements. Table X shows the network setting and requirements. \\


% \subsection{Requirement Enforcement and Scalability}
% In this set of experiments, we analyze the scalability of \system in a data center scale network and demonstrate what kind of network properties \system can verify. We consider basic requirements such as reachability and also more complex requirements including transformation and traffic engineering policies. \kerim{We discuss different DV algorithm(s) and evaluate each}

% \para{Methodology}
% We run \system on k-ary data center networks with varying k values to understand how \system's distributed verification scales with the size of the network by measuring the convergence time of the verification. In particular, we pick a set of real-world requirements and monitor the distributed verification based on a different subset of these requirements. We pick BGP as the control plane in our simulation and verify its vFIB.



% \para{Results}
% Figure~\ref{fig:scalability}
% \kerim{Expectation: convergence time increases with the $k$ (thus topology size), expecting to be non-exponential with topology size, and for each case <5 sec}


% Table~\ref{tab:requirement}. Table listing different requirements and \system's verification convergence time in seconds with different sized-and-shaped topologies. 

% \begin{figure}
% \centering
% \setlength{\abovecaptionskip}{0.1cm}
% \setlength{\belowcaptionskip}{-0.cm}
% \includegraphics[width=0.6\columnwidth]{images/reliability.png}\caption{\small{\kerim{A set of subfigures showing a) recovery time b) FCT (and/or loss rate) of TCP/UDP traffic in the network. Either two subsections for data center and arbitrary topologies or in the same figure as y parameter. y parameter also consist the topologies with same structure but different sizes. }}}\label{fig:reliability}
% %\reducespace
% %\vspace{-1.5em}
% \end{figure}

% \subsection{Reliability: Link Failure}
% \kerim{Two subsections for data center vs arbitrary topologies or in a single subsection?}
% The goal of this set of experiments consists in evaluating the
% efficacy of \system in recovering from link failures. We conduct two sets of experiments on the topologies in Figure~\ref{fig:topology} a) how fast \system recovers after a link failure compared to using a single CP b) how \system's recovery behavior affect the network traffic

% \para{Methodology}
% We considered two types of topologies a) real-word topologies (Topology Zoo) b) k-ary data center topologies. We run our experiments for real-word topologies using the emulation platform and data center topologies using ns-3 based simulation. We consider \kerim{Topology details}. We enforce a) reachability for each node b) loop-freedom. We pick the following three control planes to run in real-world topologies: an OpenFlow SDN, OSPF, and IS-IS. For the data center topologies, moreover, we run an OpenFlow SDN controller and BGP. We run UDP workloads in our evaluation \kerim{details of workload, either randomly selected pair of nodes or real-world applications from Facebook}. We randomly generate link updates in both topologies, then measure the recovery time of each control plane, flow completion time and packet loss rate for each flow.

% \para{Results}
% Figure~\ref{fig:reliability}
% \kerim{Expectations: a) for recovery time: \system recovers faster than other CPs (on average), worst case: \system recovers as the fastest recovering CP + DV delay + composition delay b) FCT/packet loss: similar expectations} 

% \subsection{Reliability: Misconfigured CPs}
% \kerim{Very similar to previous experiment but using misconfigured CPs instead of link failures}
% The goal of this set of experiments consists in evaluating the
% efficacy of \system in recovering from link failures. We conduct two sets of experiments on the topologies in Figure~\ref{fig:topology} a) how fast \system recovers after a link failure compared to using a single CP b) how \system's recovery behavior affect the network traffic

% \para{Methodology}
% We considered two types of topologies a) real-word topologies (Topology Zoo) b) k-ary data center topologies. We run our experiments for real-word topologies using the emulation platform and data center topologies using ns-3 based simulation. We consider \kerim{Topology details}. We enforce a) reachability for each node b) loop-freedom. We pick the following three control planes to run in real-world topologies: an OpenFlow SDN, OSPF, and IS-IS. For the data center topologies, moreover, we run an OpenFlow SDN controller and BGP. We run UDP workloads in our evaluation \kerim{details of workload, either randomly selected pair of nodes or real-world applications from Facebook}. We randomly generate link updates in both topologies, then measure the recovery time of each control plane, flow completion time and packet loss rate for each flow.

% \para{Results}
% Figure~\ref{fig:reliability}
% \kerim{Expectations: a) for recovery time: \system recovers faster than other CPs (on average), worst case: \system recovers as the fastest recovering CP + DV delay + composition delay b) FCT/packet loss: similar expectations} 


% \subsection{Optimizations}
% \kerim{This set of experiments is not complete yet}
% The goal of the final set of experiments is to demonstrate the benefits of optimizations in \system. The first optimization we consider is the damping mechanism on route selection, and we evaluate it by altering the link update rates on a k-ary data center network.

% \para{Methodology}

% \para{Results}


%\subsection{Large-scale simulation}














==> optimization.tex <==
\section{Practical issues}
Consistency model, stability, resource scheduling, etc.














==> outline-qiao.tex <==
//Paper layout:
Abstract+introduction: 1.25 pages
Motivation+Challenges: 1 page
Overview: 1 page
Composition framework: 1.5 pages
Distributed verification: 3 pages
Practical issues, including scheduling and discussion (on limitations): 0.75-1 page
Implementation: 0.5-0.75 page
Evaluation: 2.5-3 pages
Related work+conclusions: 0.75 page
Total: 12.25+ (12 pages limitation)

Goal: As soon as possible, write up the DV section
==== Other sections ====

==> overview.tex <==
\section{Overview}\label{sec:overview}
This section gives an overview of the key design points of \system{}, \ie, 
a distributed verification protocol and a multiple-control-plane composition, and its basic workflow.

\begin{figure}[t]
\setlength{\abovecaptionskip}{0.1cm}
\setlength{\belowcaptionskip}{-0.cm}
\centering
\includegraphics[width=\columnwidth]{images/carbide-architecture-20-v0.jpg}
\caption{\small{\system architecture.}}
\label{fig:arch}
\reducespace
\vspace{-1em}
\end{figure}


\subsection{Architecture}
\qiao{Reuse old text here, update later.} 

%The main novelties of \system lie in the new online composition layer, which dynamically composes multiple control planes to configure a single data plane, and in the enhanced data plane, which introduces a tag in each packet to record the previously visited control planes, and guarantees correctness.
In this section, we present a high-level overview of \system. We introduce its components, describe its workflow, and illustrate its capabilities. The key components of \system are shown in Figure~\ref{fig:arch}. Each network device runs (1) a control plane layer, (2) a novel online composition layer, and (3) an enhanced data plane layer. 

%At each device in \system, a composition layer is added after the control plane layer, composing multiple control planes to configure a single data plane. \red{List through all of the components of the composition layer to make it clear}
%3 layers

%\system improves network robustness while ensuring various policies by dynamically composing multiple CPs in real time.

%We consider a network as a graph $G = (V,E)$ of devices and links connecting devices.

\para{Control Plane Layer} 

The control plane layer consists of a set of control plane (CP) instances $\mathcal{CP} = \{CP_1,..., CP_k\}$ running in parallel. A control plane instance may be centralized (\eg, SDN) or distributed (\eg, OSPF). For example, a device may run three control plane instances: $CP_1$ as an SDN control plane receiving OpenFlow messages from a new release of an SDN controller, $CP_2$ as an SDN control plane receiving OpenFlow messages from  a stable release of an SDN controller, and $CP_3$ as a traditional link-state routing protocol such as OSPF.
\system treats every control plane instance as a black-box and only depends on the output (\ie, forwarding information) of each control plane instance. This design decision allows \system to use any existing implementation (open source or commercial) for each control plane instance.


%In general, a network's CP can work individually or with coordination (\eg, route redistribution) to compute the paths taken by packets to reach their destinations. We consider an ordered set of CPs $\mathcal{CP} = \{CP_1,..., CP_k\}$ such that \system in each device is capable of running a subset of $\mathcal{CP}$. The order specifies a global preference of all the CPs used by the devices.
%In the control plane layer, multiple CPs are running virtually and in parallel. Each CP can generate a dynamically-changed forwarding table (\eg, OF table or FIB) by a software process (\eg, Dijkstra algorithm for OSPF) and exchanging information ($\textcircled{1}$ in Figure) with other devices (\eg, controllers for SDN and neighbors for OSPF).

%For example, three CPs are considered: CP1 is a new SDN controller release (beta), still under testing for potential bugs; CP2 is a stable SDN controller version that the network has used for a while; CP3 is a distributed control plans running OSPF protocols. The order of the three CPs illustrates that the network should try to use the beta SDN as much as possible to test the new features; the potential bugs of beta SDN should be detected locally in the network and the stable SDN will then be used just for the affected traffic, with other traffic remains being used by beta; CP3 by OSPF is running at the bottom to guarantee connectivity under network failures, \ie, leveraging the distributed protocols to fast recover routing in the case of failures.

%\para{Correctness requirement.} Administrators specify a global network correctness requirement for each CP, denoted as $R_i$ for $CP_i$. The global requirement can be further projected to each device, denoted as $R_i(n)=projection(R_i, n)$ for device $n$. \system supports a wide range of requirement and policies, \eg, ensuring readability, waypoint traversal and ACL, etc. The formal requirement specification and projection are given later in Section.


\para{Online Composition Layer} 

This novel layer dynamically composes the information from the control plane instances to satisfy the requirements specified by an administrator. 
%This is because each control plane instance may allow a unique set of objectives to be satisfied, and forwarding every packet using a single control plane instance may be too restrictive. Instead,  we allow administrators to specify the desired policies (\eg, waypoint traversal, ACL, etc.) for the traffic, global network correctness requirements for each control plane instance, and the overall preference order between control plane instances. In the rest of this paper, we therefore assume $\mathcal{CP} = \{CP_1,..., CP_k\}$ 
%to be an ordered set, with the order specifying the global preference of the CPs. 
The online composition layer consists of four components.
\begin{itemize} [leftmargin=*]
    % Correctness Requirement Specification Point (CRSP)
    \item \textbf{\CPSpec}: This component enables administrators to specify correctness requirements (\eg, waypoint traversal, ACL, etc.) for each CP of different traffic types, and the overall preference order between control plane instances. For the rest of this paper, we consider $\mathcal{CP} = \{CP_1,..., CP_k\}$ as an ordered set of control planes from most to least preferred. Because different CPs may have different desired behavior, \CPSpec allows operators to specify \emph{different} requirements for each CP.
    
    \item \textbf{vFIB}: Each CP is associated with a virtual forwarding information base that collects and stores the forwarding information from that control plane instance.

    %    It stores the system configuration data received from administrators, including correctness requirement for each CP and CP preference. The CP correctness requirement will be formally defined in Section~\ref{}. It specifies the desired properties and constraints for a subspace of packets. For example, the new release of the SDN controller ($CP_1$) may generate configurations to enforce waypoint traversal for a set of flows. The CP preference specifies a strict order on CPs for the whole network. In the rest of this paper, we therefore assume $\mathcal{CP} = \{CP_1,..., CP_k\}$ in each device to be an ordered set, with the order specifying the global preference of the CPs. 
    \item \textbf{\DistVeri}: Each CP is also associated with \DistVeri, a light-weight event-driven verification module. Upon detecting any change in a vFIB or local forwarding state (\eg, port/link failures), \DistVeri verifies the correctness requirements for that CP in real time. For example, an administrator may specify a new release of the SDN controller ($CP_1$) to enforce specific waypoint traversal. A software bug may result in incorrect Openflow rules and fail to enforce the waypoint requirement. The goal of \DistVeri is to detect which packets have the desired correctness requirements satisfied. One key challenge for \DistVeri is that it cannot rely on a centralized entity; in the case of network partitions, a centralized entity may not be reachable. Details of the verification module are described in Section~\ref{sec:veri}. 
    \item \textbf{CP composer:} The CP composer takes as inputs the forwarding rules from the vFIBs and the verification results from the \DistVeri modules and computes the configuration to enforce at the data plane layer. 
    %One of the principles of \system is no changes to existing CPs, but the original CP rules may not be compatible with the verification results, and rules from different CPs may overlap. To this end, the CP composer in \system can generate extra CP selection rules to safely direct the traffic in the data plane to use rules from different CPs. For example, CP composer will generate a rule matches on flow $f$ and directs to the rules from vFIB2. The selection rules can also isolate the forwarding rules from different CPs, avoid rule overlapping in the single data plane. The selection rules generation is present in Section.
\end{itemize}




%\para{Verification.} In the composition layer, a light-weight verification module receives the forwarding information and updates of all the CPs ($\textcircled{2}$ in Figure), and verifies their correctness requirement in real time. The verification for different CPs are independent, thus can be executed in parallel by multiple threads. Allowing offloaded by a centralized entity though, the verification module must be able to run locally, with information exchange with neighbors ($\textcircled{3}$ in Figure). Conceptually, the verification function $(HS_i^T,HS_i^F)=Veri(CP_i,R_i(n))$ at $n$ can locally verify whether and how $CP_i$ can satisfy its requirement $R_i$. $HS_i^T$ means the subspace of packet headers ( with formal definition shown in Figure \ref{dpv-grammar}) that can satisfy, while $HS_i^F$ denotes all other packets, \ie, $HS_i^T \cap HS_i^F=\varnothing$. 
%\red{Plain English version. Forcing each device to use a single control plane is too restrictive. In our design, we assign the best possible control plane for each packet.} A naive way to verification is to verify only forwarding rules, then the $HS_i^T$ will be the union of the matches of all valid rules for $CP_i$. However, this method is too coarse-grained and provides less availability. For example, a rule matching $dstIP=D$ violates the requirement of blocking $dstPort=23$ traffic. Simply putting $dstIP=D$ in $HS_i^F$ can lead to false negative, \ie, blocking all traffic including $dstPort!=23$. The correct verification result should only include $dstIP=D\&dstPort=23$. The details of the verification module will be described in Section.

%\para{CP assignments table.} The verification results for all CPs are combined together and expressed in a table form shown as $\textcircled{4}$ in Figure. Intuitively, a packet is processed by a single CP at each device, and the CPs are in a strict order. Therefore, the device can locally downgrade to process a packet with a lower CP only if the the upper CP is not available to process it. The CP assignments table precisely specifies the CP that a packet should use, and if a packet whose header $\notin \bigcap_{i=1}^{k} HS_i^T$ will be dropped as no CPs can process the packet at device $n$ to ensure the correctness. In addition, CP assignments table can also reflect the CP usage to further guide the resource allocation in the device.

%\para{CP composition.} According to the CP assignments table, the CP composition module can generate and update the forwarding rules in the data plane ($\textcircled{5}$ in Figure). One of the principles of \system is no changes to existing CPs, so the CP composition module will selectively and transparently use forwarding rules from different CPs to compose the single data plane. However, the original CP rules may not be compatible with the verification results, and rules from different CPs may overlapping.
%To this end, the CP composition module in \system can generate extra CP selection rules according to the CP assignments table to direct the traffic in the data plane to use rules from different CPs. For example, a selection rule matching $dstIP=D\&dstPort!=23$ \footnote{Use priority to realize negation.} can direct the traffic to use forwarding rule matching $dstIP=D$ to block the none 23 traffic. The selection rules can also isolate the forwarding rules from different CPs, avoid rule overlapping in the single data plane. We implement the CP selection rules based on OF pipeline design, and the details can be found in Section.






















==> syntax.tex <==
\section{Key Syntax}
The key syntax of this grammar is explained
as follows.

\para{Header space}. A header space is specified as a predicate on packet
headers. A predicate is (1) of the form $h.f=v$ representing the set of
packets whose header field $h$ is of value $v$, or (2) the
conjunction ($\&$), disjunction ($|$) or negation ($!$) of predicates.
For example, $srcIP=10.0.1.0/24 | dstIP=10.0.2.0/24$ represents a packet space
from source IP prefix $10.0.1.0/24$ to destination IP prefix $10.0.2.0/24$.
%For simplicity, \DistVeri{} requires that different packet spaces are disjoint. This requirement
%is enforced with a pre-processor.

\para{Device-label}. \DistVeri provides a mapping from network devices to
different labels as parameters. Specifically, each device has a unique
identifier label, and multiple optional labels such as IP addresses (\eg,
10.0.0.1/24), AS number (\eg, $ASN 65533$), pod-number in a fat-tree topology
(\eg, Pod-1), and a function name (\eg, a load balancer). 

\para{Topology path set}. A path set of the topology, denoted as $P$, is
specified as (1) a regular expression whose alphabet consists of all the network
devices and a path-end symbol $\$$ or (2) the intersection ($\cap$)  or union
($\cup$) of path sets. \DistVeri also provides a syntax sugar $[label]$ to allow operators to
refer to a set of devices in a regular expression. 

%\shen{not labels, but refer to device using $[label]$; a label refers to a set of devices...}
% A regular expression that does not end with the $\$$ symbol
%means that given any path represented by this expression, the last device
%...\qiao{TBA.} is a prefix of the path,

\para{Requirement}. A requirement is specified as a tuple of a packet space $h$,  and
a set of set comparison expressions (\ie, $\subset$, $\supset$ and $=$) 
between the single-forwarding path set generated by the data plane and the path
set of the topology.
